HI aperture synthesis and optical observations of the pair of galaxies NGC 6907 and 6908

NGC 6908, a S0 galaxy situated in direction of NGC 6907, was only recently recognized as a distinct galaxy, instead of only a part of NGC 6907. We present 21 cm radio synthesis observations obtained with the GMRT and optical images and spectroscopy obtained with the Gemini North telescope of this pair of interacting galaxies. From the radio observations we obtained the velocity field and the HI column density map of the whole region containing the NGC 6907/8 pair, and by means of the Gemini multi-object spectroscopy we obtained high quality photometric images and $5 {\AA}$ resolution spectra sampling the two galaxies. By comparing the rotation curve of NGC 6907 obtained from the two opposite sides around the main kinematic axis, we were able to distinguish the normal rotational velocity field from the velocity components produced by the interaction between the two galaxies. Taking into account the rotational velocity of NGC 6907 and the velocity derived from the absorption lines for NGC 6908, we verified that the relative velocity between these systems is lower than 60 km s$^{-1}$. The emission lines observed in the direction of NGC 6908, not typical of S0 galaxies, have the same velocity expected for the NGC 6907 rotation curve. Some of them, superimposed on the absorption profiles, which reinforces the idea that they were not formed in NGC 6908. Finally, the HI profile exhibits details of the interaction, showing three components: one for NGC 6908, another for the excited gas in the NGC 6907 disk and a last one for the gas with higher relative velocities left behind NGC 6908 by dynamical friction, used to estimate the time when the interaction started in $(3.4 \pm 0.6)\times10^7$ years ago.

==> readme <==
%auto-ignore

This file contain information regarding the paper "HI aperture synthesis and 
optical observations of the pair of galaxies NGC 6907 and 6908"
Authors: S. Scarano Jr., Felipe R. H. Madsen, Nirupam Roy, J. R. D. Lepine

The contact details of the first author are as follows
S. Scarano Jr
email  : scarano@astro.iag.usp.br
    
Comments: 11 pages, 5 tables, 13 figures. Corrected typos. Accepted for 
publication in MNRAS. The definitive version will be available at 
http://www.blackwell-synergy.com .   

Abstract: NGC 6908, a S0 galaxy situated in direction of NGC 6907, was only 
recently recognized as a distinct galaxy, instead of only a part of NGC 6907. 
We present 21 cm radio synthesis observations obtained with the GMRT and 
optical images and spectroscopy obtained with the Gemini North telescope of 
this pair of interacting galaxies. From the radio observations we obtained the 
velocity field and the HI column density map of the whole region containing 
the NGC 6907/8 pair, and by means of the Gemini multi-object spectroscopy we 
obtained high quality photometric images and $5 {\AA}$ resolution spectra 
sampling the two galaxies. By comparing the rotation curve of NGC 6907 obtained 
from the two opposite sides around the main kinematic axis, we were able to 
distinguish the normal rotational velocity field from the velocity components 
produced by the interaction between the two galaxies. Taking into account the 
rotational velocity of NGC 6907 and the velocity derived from the absorption 
lines for NGC 6908, we verified that the relative velocity between these 
systems is lower than 60 km s$^{-1}$. The emission lines observed in the 
direction of NGC 6908, not typical of S0 galaxies, have the same velocity 
expected for the NGC 6907 rotation curve. Some of them, superimposed on the 
absorption profiles, which reinforces the idea that they were not formed in NGC 
6908. Finally, the HI profile exhibits details of the interaction, showing 
three components: one for NGC 6908, another for the excited gas in the NGC 6907 
disk and a last one for the gas with higher relative velocities left behind NGC 
6908 by dynamical friction, used to estimate the time when the interaction 
started in $(3.4 \pm 0.6)\times10^7$ years ago.                                                                       
                                                                                
 The compressed tar file "ngc6907.tar.gz" contain the following files:
 readme            This file
 mn2e.cls          MNRAS document class file
 mn2e.bst          MNRAS Bibliography style file 
 ngc6907.tex       TEX file of the paper 
 fig{01-13}.eps    Figure {01-13} in the paper
 00README.XXX      keepcomments file

